Acoustic Soft Tactile Skin (AST Skin)

This paper presents a novel soft tactile skin (STS) technology operating with sound waves. In this innovative approach, the sound waves generated by a speaker travel in channels embedded in a soft membrane and get modulated due to a deformation of the channel when pressed by an external force and received by a microphone at the end of the channel. The sensor leverages regression and classification methods for estimating the normal force and its contact location. Our sensor can be affixed to any robot part, e.g., end effectors or arm. We tested several regression and classifier methods to learn the relation between sound wave modulation, the applied force, and its location, respectively and picked the best-performing models for force and location predictions. Our novel tactile sensor yields 93% of the force estimation within 1.5 N tolerances for a range of 0-30+1 N and estimates contact locations with over 96% accuracy. We also demonstrated the performance of STS technology for a real-time gripping force control application.

==> parts/table2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[tb!]
\small\addtolength{\tabcolsep}{-4pt}
\centering
\caption{Comparison of various regression  models based on validation error for estimating contact force (abbreviation: SVM - Support Vector Machines, GP - Gaussian Process)}
\label{regressioncomparison}
\begin{tabular}{|lccccccccc|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Regression   models}}} & \multicolumn{9}{c|}{\textbf{STS configuration}}                                                                                                                                                                                                                                                                                   \\ \cline{2-10} 
\multicolumn{1}{|l|}{}                                              & \multicolumn{1}{c|}{\textbf{STS 1}}    & \multicolumn{1}{c|}{\textbf{STS 2a}}    & \multicolumn{1}{c|}{\textbf{STS 2b}}    & \multicolumn{1}{c|}{\textbf{STS 3a}}    & \multicolumn{1}{c|}{\textbf{STS 3b}}    & \multicolumn{1}{c|}{\textbf{STS 4a}}    & \multicolumn{1}{c|}{\textbf{STS 4b}}   & \multicolumn{1}{c|}{\textbf{STS 4c}}    & \textbf{STS 4d}    \\ \hline

\multicolumn{1}{|l|}{Linear Regression}                                        & \multicolumn{1}{c|}{2.22}          & \multicolumn{1}{c|}{5.98}          & \multicolumn{1}{c|}{7.23}          & \multicolumn{1}{c|}{4.87}          & \multicolumn{1}{c|}{2.85}          & \multicolumn{1}{c|}{7.28}          & \multicolumn{1}{c|}{7.17}         & \multicolumn{1}{c|}{5.91}          & 3.66          \\ 
\multicolumn{1}{|l|}{Interactions Linear Regression}                           & \multicolumn{1}{c|}{1.78}          & \multicolumn{1}{c|}{5.01}          & \multicolumn{1}{c|}{6.45}          & \multicolumn{1}{c|}{3.45}          & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{6.61}          & \multicolumn{1}{c|}{6.102}        & \multicolumn{1}{c|}{5.54}          & 3.13          \\ 
\multicolumn{1}{|l|}{Robust Linear Regression}                                        & \multicolumn{1}{c|}{2.54}          & \multicolumn{1}{c|}{6.33}          & \multicolumn{1}{c|}{7.74}          & \multicolumn{1}{c|}{6.13}          & \multicolumn{1}{c|}{3.81}          & \multicolumn{1}{c|}{9.17}          & \multicolumn{1}{c|}{8.29}         & \multicolumn{1}{c|}{6.72}          & 3.66          \\ 
\multicolumn{1}{|l|}{Stepwise Linear Regression}                               & \multicolumn{1}{c|}{1.78}          & \multicolumn{1}{c|}{5.01}          & \multicolumn{1}{c|}{6.46}          & \multicolumn{1}{c|}{3.46}          & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{6.61}          & \multicolumn{1}{c|}{6.11}         & \multicolumn{1}{c|}{5.54}          & 3.14          \\ \hline

\multicolumn{1}{|l|}{Fine Regression Tree}                                     & \multicolumn{1}{c|}{1.08}          & \multicolumn{1}{c|}{3.19}          & \multicolumn{1}{c|}{4.34}          & \multicolumn{1}{c|}{2.82}          & \multicolumn{1}{c|}{1.31}          & \multicolumn{1}{c|}{4.07}          & \multicolumn{1}{c|}{4.69}         & \multicolumn{1}{c|}{3.27}          & 1.59          \\ 
\multicolumn{1}{|l|}{Medium Regression Tree}                                   & \multicolumn{1}{c|}{1.18}          & \multicolumn{1}{c|}{3.02}          & \multicolumn{1}{c|}{4.26}          & \multicolumn{1}{c|}{2.62}          & \multicolumn{1}{c|}{1.24}          & \multicolumn{1}{c|}{3.86}          & \multicolumn{1}{c|}{4.5}          & \multicolumn{1}{c|}{3.1}           & 1.625         \\
\multicolumn{1}{|l|}{Coarse Regression Tree}                                   & \multicolumn{1}{c|}{1.42}          & \multicolumn{1}{c|}{3.5}           & \multicolumn{1}{c|}{4.52}          & \multicolumn{1}{c|}{2.58}          & \multicolumn{1}{c|}{1.31}          & \multicolumn{1}{c|}{4.2}           & \multicolumn{1}{c|}{4.73}         & \multicolumn{1}{c|}{3.49}          & 1.73          \\ \hline

\multicolumn{1}{|l|}{Linear SVM}                                        & \multicolumn{1}{c|}{2.4}           & \multicolumn{1}{c|}{6.1}           & \multicolumn{1}{c|}{7.52}          & \multicolumn{1}{c|}{5.39}          & \multicolumn{1}{c|}{2.94}          & \multicolumn{1}{c|}{8.09}          & \multicolumn{1}{c|}{7.41}         & \multicolumn{1}{c|}{6.18}          & 3.74          \\ 
\multicolumn{1}{|l|}{Quadratic SVM}                                     & \multicolumn{1}{c|}{1.93}          & \multicolumn{1}{c|}{5.98}          & \multicolumn{1}{c|}{6.96}          & \multicolumn{1}{c|}{3.62}          & \multicolumn{1}{c|}{2.09}          & \multicolumn{1}{c|}{7.98}          & \multicolumn{1}{c|}{5.82}         & \multicolumn{1}{c|}{5.63}          & 2.95          \\ 
\multicolumn{1}{|l|}{Cubic SVM}                                         & \multicolumn{1}{c|}{2.29}          & \multicolumn{1}{c|}{28.81}         & \multicolumn{1}{c|}{12.43}         & \multicolumn{1}{c|}{21.54}         & \multicolumn{1}{c|}{10.02}         & \multicolumn{1}{c|}{17.45}         & \multicolumn{1}{c|}{28.25}        & \multicolumn{1}{c|}{15.23}         & 24.8          \\ 
\multicolumn{1}{|l|}{Fine Gaussian SVM}                                 & \multicolumn{1}{c|}{1.04}          & \multicolumn{1}{c|}{2.42}          & \multicolumn{1}{c|}{4.34}          & \multicolumn{1}{c|}{2.319}         & \multicolumn{1}{c|}{1.3}           & \multicolumn{1}{c|}{3.31}          & \multicolumn{1}{c|}{3.7}          & \multicolumn{1}{c|}{2.95}          & 1.33          \\ 
\multicolumn{1}{|l|}{Medium Gaussian SVM}                               & \multicolumn{1}{c|}{1.24}          & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{4.26}          & \multicolumn{1}{c|}{2.73}          & \multicolumn{1}{c|}{1.52}          & \multicolumn{1}{c|}{3.96}          & \multicolumn{1}{c|}{4.5}          & \multicolumn{1}{c|}{3.98}          & 1.77          \\
\multicolumn{1}{|l|}{Coarse Gaussian SVM}                                & \multicolumn{1}{c|}{1.67}          & \multicolumn{1}{c|}{4.68}          & \multicolumn{1}{c|}{4.52}          & \multicolumn{1}{c|}{3.22}          & \multicolumn{1}{c|}{2}             & \multicolumn{1}{c|}{5.92}          & \multicolumn{1}{c|}{5.68}         & \multicolumn{1}{c|}{5.45}          & 2.78          \\ \hline



\multicolumn{1}{|l|}{Rational Quadratic GP}                            & \multicolumn{1}{c|}{0.72}          & \multicolumn{1}{c|}{\textbf{2.21}} & \multicolumn{1}{c|}{3.4}           & \multicolumn{1}{c|}{2.16}          & \multicolumn{1}{c|}{1.08}          & \multicolumn{1}{c|}{3.34}          & \multicolumn{1}{c|}{3.59}         & \multicolumn{1}{c|}{2.56}          & 1.22          \\
\multicolumn{1}{|l|}{Squared Exponential GP}                           & \multicolumn{1}{c|}{0.87}          & \multicolumn{1}{c|}{2.41}          & \multicolumn{1}{c|}{3.31}          & \multicolumn{1}{c|}{2.25}          & \multicolumn{1}{c|}{1.17}          & \multicolumn{1}{c|}{3.27}          & \multicolumn{1}{c|}{3.65}         & \multicolumn{1}{c|}{2.72}          & 1.26          \\ 
\multicolumn{1}{|l|}{Matern 5/2 GP}                                    & \multicolumn{1}{c|}{0.8}           & \multicolumn{1}{c|}{2.27}          & \multicolumn{1}{c|}{\textbf{3.24}} & \multicolumn{1}{c|}{2.2}           & \multicolumn{1}{c|}{1.14}          & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{3.6}          & \multicolumn{1}{c|}{2.61}          & 1.2           \\ 
\multicolumn{1}{|l|}{Exponential GP}                                   & \multicolumn{1}{c|}{\textbf{0.72}} & \multicolumn{1}{c|}{2.24}          & \multicolumn{1}{c|}{3.35}          & \multicolumn{1}{c|}{\textbf{2.15}} & \multicolumn{1}{c|}{\textbf{1.06}} & \multicolumn{1}{c|}{\textbf{3.25}} & \multicolumn{1}{c|}{\textbf{3.6}} & \multicolumn{1}{c|}{\textbf{2.53}} & \textbf{1.18} \\ \hline

\multicolumn{1}{|l|}{Boosted Ensemble of Trees}                                 & \multicolumn{1}{c|}{1.67}          & \multicolumn{1}{c|}{3.6}           & \multicolumn{1}{c|}{4.6}           & \multicolumn{1}{c|}{2.57}          & \multicolumn{1}{c|}{1.56}          & \multicolumn{1}{c|}{3.88}          & \multicolumn{1}{c|}{4.59}         & \multicolumn{1}{c|}{3.65}          & 1.8           \\ 
\multicolumn{1}{|l|}{Bagged Ensemble of Trees}                                  & \multicolumn{1}{c|}{0.94}          & \multicolumn{1}{c|}{2.63}          & \multicolumn{1}{c|}{3.67}          & \multicolumn{1}{c|}{2.29}          & \multicolumn{1}{c|}{1.08}          & \multicolumn{1}{c|}{3.41}          & \multicolumn{1}{c|}{3.86}         & \multicolumn{1}{c|}{2.62}          & 1.3           \\ \hline

\multicolumn{1}{|l|}{Narrow Neural Network}                                 & \multicolumn{1}{c|}{1.2}           & \multicolumn{1}{c|}{3.48}          & \multicolumn{1}{c|}{5.21}          & \multicolumn{1}{c|}{2.83}          & \multicolumn{1}{c|}{1.47}          & \multicolumn{1}{c|}{4.63}          & \multicolumn{1}{c|}{4.8}          & \multicolumn{1}{c|}{3.86}          & 1.62          \\ 
\multicolumn{1}{|l|}{Medium Neural Network}                                 & \multicolumn{1}{c|}{1.15}          & \multicolumn{1}{c|}{2.88}          & \multicolumn{1}{c|}{4.94}          & \multicolumn{1}{c|}{2.53}          & \multicolumn{1}{c|}{1.49}          & \multicolumn{1}{c|}{3.74}          & \multicolumn{1}{c|}{4.27}         & \multicolumn{1}{c|}{3.305}         & 1.51          \\ 
\multicolumn{1}{|l|}{Wide Neural Network}                           & \multicolumn{1}{c|}{1.05}          & \multicolumn{1}{c|}{2.89}          & \multicolumn{1}{c|}{4.32}          & \multicolumn{1}{c|}{2.35}          & \multicolumn{1}{c|}{1.37}          & \multicolumn{1}{c|}{3.64}          & \multicolumn{1}{c|}{3.85}         & \multicolumn{1}{c|}{2.89}          & 1.34          \\ 
\multicolumn{1}{|l|}{Bilayered Neural Network}                      & \multicolumn{1}{c|}{1.07}          & \multicolumn{1}{c|}{2.68}          & \multicolumn{1}{c|}{5.27}          & \multicolumn{1}{c|}{2.36}          & \multicolumn{1}{c|}{1.29}          & \multicolumn{1}{c|}{3.63}          & \multicolumn{1}{c|}{4.33}         & \multicolumn{1}{c|}{5.13}          & 1.41          \\
\multicolumn{1}{|l|}{Trilayered Neural Network}                     & \multicolumn{1}{c|}{0.9}           & \multicolumn{1}{c|}{2.52}          & \multicolumn{1}{c|}{4.03}          & \multicolumn{1}{c|}{2.28}          & \multicolumn{1}{c|}{1.29}          & \multicolumn{1}{c|}{3.42}          & \multicolumn{1}{c|}{3.95}         & \multicolumn{1}{c|}{2.94}          & 1.31          \\ \hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> parts/table21.tex <==
\begin{table*}[tb!]
\small\addtolength{\tabcolsep}{-4pt}
\centering
\caption{Comparison of various classifier models based on validation accuracy for estimating contact force locations (abbreviation: SVM - Support Vector Machines, K-Nearest Neighbours Algorithm)}
\label{classifiercomparison}
\begin{tabular}{|l|ccccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Classifier   Models}}} & \multicolumn{9}{c|}{\textbf{STS configuration}}                                                                                                                                                                                                                                                                                  \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                              & \multicolumn{1}{c|}{\textbf{STS 1}}    & \multicolumn{1}{c|}{\textbf{STS 2a}}    & \multicolumn{1}{c|}{\textbf{STS 2b}}    & \multicolumn{1}{c|}{\textbf{STS 3a}}    & \multicolumn{1}{c|}{\textbf{STS 3b}}    & \multicolumn{1}{c|}{\textbf{STS 4a}}    & \multicolumn{1}{c|}{\textbf{STS 4b}}    & \multicolumn{1}{c|}{\textbf{STS 4c}}    & \textbf{STS 4d}    \\ \hline

Fine Tree                                                           & \multicolumn{1}{c|}{91.3}          & \multicolumn{1}{c|}{93.2}          & \multicolumn{1}{c|}{95}            & \multicolumn{1}{c|}{90.5}          & \multicolumn{1}{c|}{86.1}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{95.6}          & 93.9          \\ 
Medium Tree                                                         & \multicolumn{1}{c|}{78.8}          & \multicolumn{1}{c|}{92.9}          & \multicolumn{1}{c|}{85.8}          & \multicolumn{1}{c|}{87.6}          & \multicolumn{1}{c|}{74.2}          & \multicolumn{1}{c|}{85.7}          & \multicolumn{1}{c|}{90.1}          & \multicolumn{1}{c|}{94.8}          & 78.5          \\ 
Coarse Tree                                                         & \multicolumn{1}{c|}{69.9}          & \multicolumn{1}{c|}{87.1}          & \multicolumn{1}{c|}{71}            & \multicolumn{1}{c|}{74.5}          & \multicolumn{1}{c|}{60.2}          & \multicolumn{1}{c|}{77.1}          & \multicolumn{1}{c|}{84.2}          & \multicolumn{1}{c|}{87.6}          & 67            \\ \hline

Linear Discriminant                                                 & \multicolumn{1}{c|}{70.7}          & \multicolumn{1}{c|}{89.4}          & \multicolumn{1}{c|}{89.2}          & \multicolumn{1}{c|}{74.8}          & \multicolumn{1}{c|}{59}            & \multicolumn{1}{c|}{79}            & \multicolumn{1}{c|}{82.1}          & \multicolumn{1}{c|}{70.4}          & 73.5          \\ 
Quadratic Discriminant                                              & \multicolumn{1}{c|}{70.3}          & \multicolumn{1}{c|}{89}            & \multicolumn{1}{c|}{89.5}          & \multicolumn{1}{c|}{79}            & \multicolumn{1}{c|}{58.4}          & \multicolumn{1}{c|}{80.6}          & \multicolumn{1}{c|}{88}            & \multicolumn{1}{c|}{88}            & 87.3          \\ \hline
 
Guassian Naïve Bayes                                                & \multicolumn{1}{c|}{42.2}          & \multicolumn{1}{c|}{73.9}          & \multicolumn{1}{c|}{72.7}          & \multicolumn{1}{c|}{46.3}          & \multicolumn{1}{c|}{39.2}          & \multicolumn{1}{c|}{74}            & \multicolumn{1}{c|}{79.2}          & \multicolumn{1}{c|}{63.8}          & 60.9          \\ 
Kernal Naïve Bayes                                                  & \multicolumn{1}{c|}{72.6}          & \multicolumn{1}{c|}{84.2}          & \multicolumn{1}{c|}{78.1}          & \multicolumn{1}{c|}{77.2}          & \multicolumn{1}{c|}{61.9}          & \multicolumn{1}{c|}{77.3}          & \multicolumn{1}{c|}{86.6}          & \multicolumn{1}{c|}{89.7}          & 73.9          \\ \hline

Linear SVM                                                              & \multicolumn{1}{c|}{77.2}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{88.5}          & \multicolumn{1}{c|}{78.4}          & \multicolumn{1}{c|}{62.7}          & \multicolumn{1}{c|}{84.4}          & \multicolumn{1}{c|}{86}            & \multicolumn{1}{c|}{83.4}          & 84.4          \\ 
Quadratic SVM                                                           & \multicolumn{1}{c|}{94.3}          & \multicolumn{1}{c|}{91.9}          & \multicolumn{1}{c|}{93.5}          & \multicolumn{1}{c|}{90.2}          & \multicolumn{1}{c|}{61.1}          & \multicolumn{1}{c|}{88}            & \multicolumn{1}{c|}{93.6}          & \multicolumn{1}{c|}{96.1}          & 89.1          \\ 
Cubic SVM                                                               & \multicolumn{1}{c|}{72}            & \multicolumn{1}{c|}{65.9}          & \multicolumn{1}{c|}{95.7}          & \multicolumn{1}{c|}{48.2}          & \multicolumn{1}{c|}{53.2}          & \multicolumn{1}{c|}{64.5}          & \multicolumn{1}{c|}{60.8}          & \multicolumn{1}{c|}{71.8}          & 74.9          \\ 
Fine Guassian SVM                                                       & \multicolumn{1}{c|}{96}            & \multicolumn{1}{c|}{\textbf{95.7}} & \multicolumn{1}{c|}{98.1}          & \multicolumn{1}{c|}{92.2}          & \multicolumn{1}{c|}{87.8}          & \multicolumn{1}{c|}{92.6}          & \multicolumn{1}{c|}{\textbf{95.4}} & \multicolumn{1}{c|}{97.2}          & 97.1          \\
Medium Guassian SVM                                                   & \multicolumn{1}{c|}{94.4}          & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{93}            & \multicolumn{1}{c|}{91.3}          & \multicolumn{1}{c|}{81.3}          & \multicolumn{1}{c|}{91.2}          & \multicolumn{1}{c|}{93.8}          & \multicolumn{1}{c|}{95.9}          & 93.2          \\ 
Coarse Guassian SVM                                                    & \multicolumn{1}{c|}{74.4}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{88.7}          & \multicolumn{1}{c|}{88.5}          & \multicolumn{1}{c|}{63.9}          & \multicolumn{1}{c|}{85.6}          & \multicolumn{1}{c|}{89.1}          & \multicolumn{1}{c|}{86.8}          & 87.5          \\ \hline

Fine KNN                                                            & \multicolumn{1}{c|}{95}            & \multicolumn{1}{c|}{94.5}          & \multicolumn{1}{c|}{97.7}          & \multicolumn{1}{c|}{90.2}          & \multicolumn{1}{c|}{89.3}          & \multicolumn{1}{c|}{91.2}          & \multicolumn{1}{c|}{93.7}          & \multicolumn{1}{c|}{96.6}          & 96.6          \\ 
Medium KNN                                                          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{95.4}          & \multicolumn{1}{c|}{98}            & \multicolumn{1}{c|}{92.1}          & \multicolumn{1}{c|}{91}            & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{97}            & 97.3          \\ 
Coarse KNN                                                          & \multicolumn{1}{c|}{82.7}          & \multicolumn{1}{c|}{93.4}          & \multicolumn{1}{c|}{93.4}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{81}            & \multicolumn{1}{c|}{91.1}          & \multicolumn{1}{c|}{93.2}          & \multicolumn{1}{c|}{93.6}          & 92.7          \\ 
Cosine KNN                                                          & \multicolumn{1}{c|}{86.6}          & \multicolumn{1}{c|}{93.7}          & \multicolumn{1}{c|}{95.5}          & \multicolumn{1}{c|}{90}            & \multicolumn{1}{c|}{85.3}          & \multicolumn{1}{c|}{89.4}          & \multicolumn{1}{c|}{92.6}          & \multicolumn{1}{c|}{89.2}          & 90.7          \\ 
Cubic KNN                                                           & \multicolumn{1}{c|}{94.4}          & \multicolumn{1}{c|}{95.3}          & \multicolumn{1}{c|}{98}            & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{90.6}          & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{97}            & 97.2          \\ 
Weighted KNN                                                        & \multicolumn{1}{c|}{95.8}          & \multicolumn{1}{c|}{95.6}          & \multicolumn{1}{c|}{\textbf{98.2}} & \multicolumn{1}{c|}{92.1}          & \multicolumn{1}{c|}{91}            & \multicolumn{1}{c|}{\textbf{92.8}} & \multicolumn{1}{c|}{94.8}          & \multicolumn{1}{c|}{\textbf{97.2}} & \textbf{97.3} \\ \hline

Boosted Ensemble Trees                                                       & \multicolumn{1}{c|}{82.7}          & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{90.4}          & \multicolumn{1}{c|}{75.8}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{92.7}          & \multicolumn{1}{c|}{96}            & 91.1          \\ 
Bagged Ensemble Trees                                                        & \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{95.4}          & \multicolumn{1}{c|}{97.6}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{\textbf{91.9}} & \multicolumn{1}{c|}{92.6}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{96.9}          & 96.8          \\ 
Subspace Discriminant                                               & \multicolumn{1}{c|}{50.9}          & \multicolumn{1}{c|}{78.4}          & \multicolumn{1}{c|}{85.3}          & \multicolumn{1}{c|}{60.8}          & \multicolumn{1}{c|}{49.7}          & \multicolumn{1}{c|}{75.4}          & \multicolumn{1}{c|}{84.1}          & \multicolumn{1}{c|}{66.9}          & 74.1          \\ 
Subspace Ensemble KNN                                                        & \multicolumn{1}{c|}{89.7}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{90}            & \multicolumn{1}{c|}{84.1}          & \multicolumn{1}{c|}{82.1}          & \multicolumn{1}{c|}{85.4}          & \multicolumn{1}{c|}{86}            & \multicolumn{1}{c|}{92.7}          & 91.4          \\ 
RUSBossted Ensemble Trees                                                    & \multicolumn{1}{c|}{78.8}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{85.8}          & \multicolumn{1}{c|}{87.6}          & \multicolumn{1}{c|}{74.2}          & \multicolumn{1}{c|}{85.7}          & \multicolumn{1}{c|}{90.1}          & \multicolumn{1}{c|}{94.9}          & 78.5          \\  \hline

Narrow Neural Network                                                           & \multicolumn{1}{c|}{95.6}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{96.9}          & \multicolumn{1}{c|}{91.7}          & \multicolumn{1}{c|}{86.7}          & \multicolumn{1}{c|}{92.2}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{96.9}          & 95.8          \\ 
Medium Neural Network                                                           & \multicolumn{1}{c|}{96.3}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{97.8}          & \multicolumn{1}{c|}{92.3}          & \multicolumn{1}{c|}{89.4}          & \multicolumn{1}{c|}{92.5}          & \multicolumn{1}{c|}{95.3}          & \multicolumn{1}{c|}{97.1}          & 97.2          \\ 
Wide Neural Network                                                             & \multicolumn{1}{c|}{96.1}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{97.6}          & \multicolumn{1}{c|}{92.2}          & \multicolumn{1}{c|}{90.3}          & \multicolumn{1}{c|}{92.5}          & \multicolumn{1}{c|}{94}            & \multicolumn{1}{c|}{97}            & 96.8          \\ 
Bilayered Neural Network                                                        & \multicolumn{1}{c|}{96.2}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{97.2}          & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{89}            & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{96.9}          & 96.9          \\ 
Trilayered Neural Network                                                       & \multicolumn{1}{c|}{95.8}          & \multicolumn{1}{c|}{95.1}          & \multicolumn{1}{c|}{97.6}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{89.3}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{94.5}          & \multicolumn{1}{c|}{97.2}          & 97            \\ \hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> parts/table3old.tex <==
\begin{table}[t!]
\small\addtolength{\tabcolsep}{-4pt}
\begin{center}
\caption{Predicted location of contact force}
\label{contactprediction}
\begin{tabular}{|c|ccc|c|}
\hline
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{AST-skin}\\ \textbf{configuration}\end{tabular}} & \multicolumn{3}{c|}{\textbf{True predictions}}                  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Accuracy}\\ (\%)\end{tabular}} \\ \cline{2-4}
              & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{B} & C &      \\ \hline
AST 1                  & \multicolumn{1}{l|}{169}  &\multicolumn{1}{l|}{160}  &164   & 96.66          \\ \hline
AST2a                 & \multicolumn{1}{l|}{169}  & \multicolumn{1}{l|}{168}  &153   & 96.07            \\ \hline
AST2b                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{169}  &168   & 99.01            \\ \hline
AST3a                 & \multicolumn{1}{l|}{165}  & \multicolumn{1}{l|}{150}  &161   & 93.33            \\ \hline
AST3b                 & \multicolumn{1}{l|}{163}  & \multicolumn{1}{l|}{142}  &150   & 89.21            \\ \hline
AST4a                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{151}  &155   &  92.94           \\ \hline
AST4b                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{156}  &162   & 95.29            \\ \hline
AST4c                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{165}  &166   & 97.84            \\ \hline
AST4d                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{167}  &162   & 97.45   \\ \hline
\end{tabular}
\end{center}
\end{table}



\iffalse
\begin{table}[t!]
\small\addtolength{\tabcolsep}{-4pt}
\begin{center}
\caption{Predicted location of contact force}
\label{contactprediction}
\begin{tabular}{|c|ccc|c|}
\hline
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{AST-skin}\\ \textbf{configuration}\end{tabular}} & \multicolumn{3}{c|}{\textbf{True predictions}}                  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Accuracy}\\ (\%)\end{tabular}} \\ \cline{2-4}
              & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{B} & C &      \\ \hline
AST 1                  & \multicolumn{1}{l|}{169}  &\multicolumn{1}{l|}{160}  &164   & 96.66          \\ \hline
AST2a                 & \multicolumn{1}{l|}{169}  & \multicolumn{1}{l|}{168}  &153   & 96.07            \\ \hline
AST2b                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{169}  &168   & 99.01            \\ \hline
AST3a                 & \multicolumn{1}{l|}{165}  & \multicolumn{1}{l|}{150}  &161   & 93.33            \\ \hline
AST3b                 & \multicolumn{1}{l|}{163}  & \multicolumn{1}{l|}{142}  &150   & 89.21            \\ \hline
AST4a                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{151}  &155   &  92.94           \\ \hline
AST4b                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{156}  &162   & 95.29            \\ \hline
AST4c                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{165}  &166   & 97.84            \\ \hline
AST4d                 & \multicolumn{1}{l|}{168}  & \multicolumn{1}{l|}{167}  &162   & 97.45   \\ \hline
\end{tabular}
\end{center}
\end{table}
\fi
